Sharp Guarantees for Solving Random Equations with One-Bit Information

We study the performance of a wide class of convex optimization-based estimators for recovering a signal from corrupted one-bit measurements in high-dimensions. Our general result predicts sharply the performance of such estimators in the linear asymptotic regime when the measurement vectors have entries IID Gaussian. This includes, as a special case, the previously studied least-squares estimator and various novel results for other popular estimators such as least-absolute deviations, hinge-loss and logistic-loss. Importantly, we exploit the fact that our analysis holds for generic convex loss functions to prove a bound on the best achievable performance across the entire class of estimators. Numerical simulations corroborate our theoretical findings and suggest they are accurate even for relatively small problem dimensions.

==> app.tex <==
\appendix
%\section{Useful properties of Prox}
%
%\begin{propo} For a function $\ell:\R\rightarrow\R$, and all $x\in\R$ and $\lambda>0$, the following properties are true
%
%
%{(i).}~~~~~ $e_{\ell,1}^{'}(x,\la) = \frac{1}{\la}{(x-\prox{x}{\la})} = \elld(\proxl{x}{\la},$
%
%{(ii).}~~~~~ $e_{\ell,2}^{'}(x,\la) = -\frac{1}{2\la^2}{(x-\prox{x}{\la})^2} = -\frac{1}{2}(\elld(\proxl{x}{\la})^2,$
%
%\end{propo}
%% proof of lemma
\begin{remark}[Upper bound on correlation]
We use the result of Theorem \ref{thm:main} to derive an upper bound on the correlation value $\corr{\xh_\ell}{\x_0}$ that holds for all choices of continuously differentiable loss functions. For simplicity, we focus on the noiseless case (i.e., $\eps=0$ in \eqref{eq:gen_model}, and defer the general case to the long version of the paper. An interesting important direction for future work is to study whether the  bound of the lemma can be attained by certain loss function.
Thus, we see that Theorem \ref{thm:main} can be useful for the design of optimal loss functions in \eqref{eq:gen_opt}.
\begin{lem}[Upper bound] Let $\ell$ be continuously differentiable and let the assumptions and notation of Theorem \ref{thm:main} hold. Fix $\eps=0$ in \eqref{eq:gen_model}. Then, 
$$
\lim_{n\rightarrow+\infty}\,\corr{\xh_\ell}{\x_0}\,\leq\, {\color{red}????} %\sqrt{1-\frac{1}{\delta}}\,.
$$
\Christos{Check!!!}
\end{lem}
\begin{proof} In view of \eqref{eq:corr_thm}, it suffices to lower bound the ratio $\sig_\ell:=\alpha/\mu$.

First, applying Gaussian integration by parts in \eqref{eq:lambda_main} we find that $$1=\lambda\, \delta\,\E[\envddx{\ell}{\ourx}{\la}],$$
where $\envddx{\ell}{x}{\la}$ denotes the second derivative of the Moreau-envelope function with respect to the first argument (which exists since $\ell$ is differentiable). Solving for $\lambda$ and substituting in \eqref{eq:alpha_main} gives 
\bea\label{eq:lower}
\alpha^2 = \frac{1}{\delta}\cdot\frac{ \E\left[\left(\envdx{\ell}{\ourx}{\la}\right)^2\right] }{\left(\,\E[\envddx{\ell}{\ourx}{\la}]\,\right)^2}.
\eea
The rest of the proof follows steps similar to \cite[Lem.~3.4]{MontanariHigh} and \cite[Rem.~5.3.3]{Master}. 
Call $$Z:=\mu S Y=\mu |S|\quad\text{and}\quad H:=\alpha G + Z.$$ Also, for a random variable $W$ with density $p_W(w)$ that has a derivative $p_W(w)$ for \emph{every} $w$, denote its score function $\ksi_w:=\frac{\partial}{\partial w}{\log p(w)}=\frac{p_W^{'}(w)}{p_W(w)}$ and consider the Fisher information (for the location family) of $W$, (e.g., \cite[Sec.~2]{barron1984monotonic})
$$
\Ic(W):=\Exp[\,(\ksi_W)^2\,].
$$
Note that for $\alpha\neq 0$ $H$ has a continuously differentiable function at every $h$; in fact,
$$
p_H^{'}(h) = \int \phi_{\alpha}^{'}(u) p_{Z}(h-u)\, \mathrm{d}u,
$$
where $\phi_{\alpha}(u)=\frac{1}{\alpha\sqrt{2\pi}}e^{-\frac{u^2}{2\alpha^2}}$.

With this notation, by Cauchy-Schwartz inequality we have 
\begin{align*}
\E\left[\left(\envdx{\ell}{H}{\la}\right)^2\right]\cdot \Ic(H) 
&\geq\left(\E[\envdx{\ell}{H}{\la}\cdot \ksi_H]\right)^2\\
&=\left(\E[\envddx{\ell}{H}{\la}]\right)^2,
\end{align*}
where the last line follows by integration by parts.
This, when combined with \eqref{eq:lower} shows that 
\bea\label{eq:lower2}
\alpha^2 \geq \frac{1}{\delta}\cdot \frac{1}{\Ic(H)}.
\eea
Recall that $H=\alpha G + \mu |S|$ and $G\sim\Nn(0,1)$. Now, since (e.g., \cite[Eqn.~2.13]{barron1984monotonic})
$$
\Ic(c\cdot W) = \Ic(W)/c^2,
$$
we have that
$$
\Ic(H) = \Ic\left(\mu \,\Big(\frac{\alpha}{\mu} G + |S| \Big)\right) = \frac{1}{\mu^2}\Ic\big(\sig_\ell\, G + |S|\big),
$$
where recall that 
$$
\sig_\ell := \alpha\big/\mu.
$$
Substituting this in \eqref{eq:lower2}, we find that
\bea\label{eq:lower2}
\sig_\ell^2 \geq \frac{1}{\delta}\cdot \frac{1}{\Ic\big(\sig_\ell\, G + |S|\big)}.
\eea
{\color{red}To complete the proof, it remains to upper bound $\Ic\big(\sig_\ell\, G + |S|\big)$.}

\Christos{That shouldn't be so hard to do!!! However, the approach (see below) that I know of and would use fails. I think up to here we are good though.} 

If $|S|$ (or more generally for the noisy case $Y\,S$) had an \emph{everywhere} continuously differentiable density then, we could use Stam's convolution inequality for Fisher information \cite{blachman1965convolution}
$$
\Ic(X+W)\leq \frac{\Ic(X)\Ic(W)}{\Ic(X)+\Ic(W)}.
$$
For $X=\sig_\ell \,G$, we have $\Ic(X)=\sig_\ell^{-2}$. Thus
\bea\label{eq:Stam}
\Ic(\sig_\ell \,G+W)\leq \frac{\Ic(W)}{1+\sig_\ell^2\Ic(W)}.
\eea
Applying this for $W=S\cdot Y$ and using it in \eqref{eq:lower2}, we would find that
\bea\label{eq:lower}
\sig_\ell^2 \geq \frac{1}{\delta-1}.
\eea
\Christos{But this lower bound violates the quadratic loss (at least for the noiseless case that we checked), so it is wrong. Is the mistake that I can't apply \eqref{eq:Stam} since $Y\, S$ does not have a derivative everywhere??}

\Christos{Perhaps we don't need that "fancy" Stam's inequality here to get an upper bound on $\Ic\big(\sig_\ell\, G + |S|\big)$ because $G,S$ are simple Gaussians and we sort of know the density of their sum.}
%
%To finish the proof of the lemma recall that $Z=\mu |Y|$; direct calculation shows that $\Ic_Z=\mu^2$.
% $\Ic_Z=(2-2/\pi)\,\mu^2.$ \Christos{Check!!!}. 
% The last step is to apply \eqref{eq:lower} in \eqref{eq:corr_thm}.
\end{proof}
\end{remark}

\begin{remark}[Why $\delta>1$] The theorem assumes that $\delta>1$ or equivalently that $m>n$. Here, we show that this condition is \emph{necessary} for the equations \eqref{eq:eq_main} to have a bounded solution, or equivalently for the minimizer $\xh_\ell$ in \eqref{eq:gen_opt} to be bounded.
%\begin{lem} If the Equations  \eqref{eq:eq_main} have a bounded solution, then $\delta>1$.
%\end{lem}
%\begin{proof}
To see this, take squares in both sides of \eqref{eq:lambda_main} and divide by \eqref{eq:alpha_main}, to find that 
$$
\delta = \frac{\Exp\left[\,\left(\envdx{\ell}{\ourx}{\la}\right)^2\,\right]}{\E\left[ G\cdot \envdx{\ell}{\ourx}{\la} \right]} \geq 1.
$$
The inequality follows by applying Cauchy-Schwarz and using the fact that $\E[G^2]=1$. To continue, 
%\end{proof}
\end{remark}
%%proof 


\subsection{Proof of \eqref{eq:Stam}} \label{sec:upperboundstam}\begin{proof}
Let $Z = \sigma_{\ell}G + |S|$. Moreover let $p(x), q(y)$ and $r(z)$ denote the probability distributions of $\sigma_{\ell}G, |S|$ and $Z$, respectively. then:
\bea
r'(z) = \int_{-\infty}^{\infty} p'(x)q(z-x)dx.\nonumber
\eea
Thus
\bea
\frac{r'(z)}{r(z)} &= \int_{-\infty}^{\infty} \frac{p(x)q(z-x)}{r(z)}\frac{p'(x)}{p(x)}dx \nonumber \\ 
&=\mathbb{E}\left[\frac{p'(x)}{p(x)} \Bigg| z\right].\nonumber
\eea
Similarly,
\bea
\frac{r'(z)}{r(z)} = \mathbb{E}\left[\frac{q'(|y|)}{q(|y|)} \Bigg | z\right].\nonumber
\eea
Therefore for any constants a and b,
\bea
\mathbb{E}\left[a\frac{p'(x)}{p(x)} + b\frac{q'(|y|)}{q(|y|)}\Bigg | z\right ] = (a+b)\frac{r'(z)}{r(z)}\nonumber
\eea
Subsequently,
\bea \label{eq:secondmoment}
(a+b)^2 \left(\frac{r'(z)}{r(z)}\right)^2 &= \left(\mathbb{E}\left[a\frac{p'(x)}{p(x)} + b\frac{q'(|y|)}{q(|y|)}\Bigg | z\right ] \right)^2 \nonumber \\
& \le \mathbb{E}\left[\left(a\frac{p'(x)}{p(x)} + b\frac{q'(|y|)}{q(|y|)}\right)^2\Bigg | z\right ] 
\eea
Taking expectation with respect to $z$ from both sides of \eqref{eq:secondmoment} gives:
\bea
(a+b)^2 &\mathbb{E}\left[\left(\frac{r'(z)}{r(z)}\right)^2\right] \le \mathbb{E}\left[\left(a\frac{p'(x)}{p(x)} + b\frac{q'(|y|)}{q(|y|)}\right)^2\right ] \nonumber \\
&=a^2\mathbb{E}\left[\left(\frac{p'(x)}{p(x)}\right)^2\right] + b^2\mathbb{E}\left[\left(\frac{q'(|y|)}{q(|y|)}\right)^2\right],\label{eq:fi}
\eea
where the last line follows from $\mathbb{E}\left[\frac{p'(x)}{p(x)}\right]=0$ and
independence of two random variables $G$ and $S$.\\
Recalling the definition of fisher information, the following inequality is derived from \eqref{eq:fi}:
 \bea
(a+b)^2 \Ic(Z) &\le a^2 \Ic(\sigma_{\ell}G) + 2b^2\Ic(|S|)\nonumber\\
&= \frac{a^2}{\sigma_{\ell}^2}+2b^2 \label{eq:beforeopt}
\eea
Setting $a=\sigma_{\ell}^2$ and $b=\frac{1}{2}$ in \eqref{eq:beforeopt} results in:
\bea
\Ic(Z) \le \frac{2}{1+2\sigma_{\ell}^2}\nonumber
\eea
\end{proof}
%% remark

\begin{remark}[Upper bound on correlation]
We use the result of Theorem \ref{thm:main} to derive an upper bound on the correlation value $\corr{\xh_\ell}{\x_0}$ that holds for all choices of continuously differentiable loss functions. For simplicity, we focus on the noiseless case (i.e., $\eps=0$ in \eqref{eq:gen_model}). An interesting important direction for future work is to study whether the  bound of the lemma can be attained by certain loss function.
Thus, we see that Theorem \ref{thm:main} can be useful for the design of optimal loss functions in \eqref{eq:gen_opt}.
\begin{lem}[Upper bound] Let $\ell$ be continuously differentiable and let the assumptions and notation of Theorem \ref{thm:main} hold. Fix $\eps=0$ in \eqref{eq:gen_model}. Then, 
$$
\lim_{n\rightarrow+\infty}\,\corr{\xh_\ell}{\x_0}\,\leq\, {\color{red}\frac{1}{\sqrt{1+\frac{1}{2(\delta-1)}}}} %\sqrt{1-\frac{1}{\delta}}\,.
$$
{\color{red},Hossein: I think Blachman's approach can be extended to our problem, please check appendix E for the proof}
\end{lem}
\begin{proof} In view of \eqref{eq:corr_thm}, it suffices to lower bound the ratio $\sig_\ell:=\alpha/\mu$.

First, applying Gaussian integration by parts in \eqref{eq:lambda_main} we find that $$1=\lambda\, \delta\,\E[\envddx{\ell}{\ourx}{\la}],$$
where $\envddx{\ell}{x}{\la}$ denotes the second derivative of the Moreau-envelope function with respect to the first argument (which exists since $\ell$ is differentiable). Solving for $\lambda$ and substituting in \eqref{eq:alpha_main} gives 
\bea\label{eq:lower}
\alpha^2 = \frac{1}{\delta}\cdot\frac{ \E\left[\left(\envdx{\ell}{\ourx}{\la}\right)^2\right] }{\left(\,\E[\envddx{\ell}{\ourx}{\la}]\,\right)^2}.
\eea
The rest of the proof follows steps similar to \cite[Lem.~3.4]{MontanariHigh} and \cite[Rem.~5.3.3]{Master}. 
Call $$Z:=\mu S Y=\mu |S|\quad\text{and}\quad H:=\alpha G + Z.$$ Also, for a random variable $W$ with density $p_W(w)$ that has a derivative $p_W(w)$ for \emph{every} $w$, denote its score function $\ksi_w:=\frac{\partial}{\partial w}{\log p(w)}=\frac{p_W^{'}(w)}{p_W(w)}$ and consider the Fisher information (for the location family) of $W$, (e.g., \cite[Sec.~2]{barron1984monotonic})
$$
\Ic(W):=\Exp[\,(\ksi_W)^2\,].
$$
Note that for $\alpha\neq 0$ $H$ has a continuously differentiable function at every $h$; in fact,
$$
p_H^{'}(h) = \int \phi_{\alpha}^{'}(u) p_{Z}(h-u)\, \mathrm{d}u,
$$
where $\phi_{\alpha}(u)=\frac{1}{\alpha\sqrt{2\pi}}e^{-\frac{u^2}{2\alpha^2}}$.

With this notation, by Cauchy-Schwartz inequality we have:
\begin{align*}
\E\left[\left(\envdx{\ell}{H}{\la}\right)^2\right]\cdot \Ic(H) 
&\geq\left(\E[\envdx{\ell}{H}{\la}\cdot \ksi_H]\right)^2\\
&=\left(\E[\envddx{\ell}{H}{\la}]\right)^2,
\end{align*}
where the last line follows by integration by parts.
This, when combined with \eqref{eq:lower} shows that: 
\bea\label{eq:lower2}
\alpha^2 \geq \frac{1}{\delta}\cdot \frac{1}{\Ic(H)}.
\eea
Recall that $H=\alpha G + \mu |S|$ and $G\sim\Nn(0,1)$. Now, since (e.g., \cite[Eqn.~2.13]{barron1984monotonic})
$$
\Ic(c\cdot W) = \Ic(W)/c^2,
$$
we have that
$$
\Ic(H) = \Ic\left(\mu \,\Big(\frac{\alpha}{\mu} G + |S| \Big)\right) = \frac{1}{\mu^2}\Ic\big(\sig_\ell\, G + |S|\big),
$$
where recall that 
$$
\sig_\ell := \alpha\big/\mu.
$$
Substituting this in \eqref{eq:lower2}, we find that
\bea\label{eq:lower3}
\sig_\ell^2 \geq \frac{1}{\delta}\cdot \frac{1}{\Ic\big(\sig_\ell\, G + |S|\big)}.
\eea
%{\color{red}To complete the proof, it remains to upper bound $\Ic\big(\sig_\ell\, G + |S|\big)$.}

%\Christos{That shouldn't be so hard to do!!! However, the approach (see below) that I know of and would use fails. I think up to here we are good though.} 

%If $|S|$ (or more generally for the noisy case $Y\,S$) had an \emph{everywhere} continuously differentiable density then, we could use Stam's convolution inequality for Fisher information \cite{blachman1965convolution}
Next we use the following upper bound (refer to Appendix \ref{sec:upperboundstam} for the proof)
%\bea\label{eq:upperboundstam}
%\Ic(X+W)\leq \frac{2\Ic(X)\Ic(W)}{\Ic(X)+2\Ic(W)}.
%\eea
%For $X=\sig_\ell \,G$, we have $\Ic(X)=\sig_\ell^{-2}$. Thus
\bea\label{eq:Stam}
\Ic(\sig_\ell \,G+|S|)\leq \frac{2}{1+2\sig_\ell^2}.
\eea
Combining \eqref{eq:lower3} and \eqref{eq:Stam} gives:
%Applying this for $W=S\cdot Y$ and using it in \eqref{eq:lower2}, we would find that:
\bea\label{eq:lower4}
\sig_\ell^2 \geq \frac{1}{2} \frac{1}{\delta-1}.
\eea
The desired inequality follows directly from  \eqref{eq:lower4}
%\Christos{But this lower bound violates the quadratic loss (at least for the noiseless case that we checked), so it is wrong. Is the mistake that I can't apply \eqref{eq:Stam} since $Y\, S$ does not have a derivative everywhere??}

%\Christos{Perhaps we don't need that "fancy" Stam's inequality here to get an upper bound on $\Ic\big(\sig_\ell\, G + |S|\big)$ because $G,S$ are simple Gaussians and we sort of know the density of their sum.}
%
%To finish the proof of the lemma recall that $Z=\mu |Y|$; direct calculation shows that $\Ic_Z=\mu^2$.
% $\Ic_Z=(2-2/\pi)\,\mu^2.$ \Christos{Check!!!}. 
% The last step is to apply \eqref{eq:lower} in \eqref{eq:corr_thm}.
\end{proof}
\end{remark}



